Everything old is new again: A multi-view learning approach to learning using privileged information and distillation

We adopt a multi-view approach for analyzing two knowledge transfer settings---learning using privileged information (LUPI) and distillation---in a common framework. Under reasonable assumptions about the complexities of hypothesis spaces, and being optimistic about the expected loss achievable by the student (in distillation) and a transformed teacher predictor (in LUPI), we show that encouraging agreement between the teacher and the student leads to reduced search space. As a result, improved convergence rate can be obtained with regularized empirical risk minimization.

==> _region_.tex <==
\message{ !name(algorithm1.tex)}
\message{ !name(algorithm1.tex) !offset(-2) }
\subsection{Analysis for learning with priviledged information}
In the case of learning with priviledged information, the two views $\x$
and $\z$ are different, and the correlation between them comes into play
when transfering priviledged information from $\z$ to $\x$. 

Perform the following change of coordinates (recall that $\tU$ and $\tV$ have full dimensions and thus these new variables are well defined): 
\begin{align*}
\tx  & = \tU^\top \x \in \bbR^{d_x}, 
\qquad\quad \tz  = \tV^\top  \z \in \bbR^{d_z}, \\
\tw & = \tU^\top \w \in \bbR^{d_x},
\qquad\quad \tv  = \tV^\top \vv \in \bbR^{d_z}.
\end{align*} 
Clearly, the transformed data has identity covariance, \ie, $\bbE \sbr{\tx \tx^\top} = \I$ and $\bbE \sbr{\tz \tz^\top} = \I$.
On the other hand, we have $\tw^\top \tx = \w^\top \x$ and $\tv^\top \tz = \vv^\top \z$.
% Based on our assumptions, we have $\norm{\tx} = \norm{\x} \le R$.

Based on the above coordinate transformation and the definition of CCA, an important observation made by Kakade et al is the following equality.
\begin{lem}[Lemma~2 of~\citet{KakadeFoster07a} re-stated]
\label{lem:agreement-as-regularizer}
For any $\w \in \bbR^{d_x}$ and $\vv \in \bbR^{d_y}$, we have
\begin{align*}
\bbE \norm{\w^\top \x - \vv^\top \z}^2
& = \sum_{i=1}^{d_x} (1-\lambda_i)  (\tw^i)^2 + \sum_{i=1}^{r} \lambda_i (\tw^i - \tv^i)^2 + \sum_{i=1}^{d_z} (1-\lambda_i) (\tv^i)^2
\\
& =  \sum_{i=1}^{d_x} (\tw^i - \lambda_i \tv^i)^2 + \sum_{i=1}^{d_z} (1-\lambda_i^2) (\tv^i)^2,
\end{align*}
with the convention that $\lambda_i=0$ for $i>rank(\Exz)$, and that $\tv^i=0$ for $i>d_z$.
\end{lem}
This lemma implies, for a pair of predictors $(\w,\vv)$ that agree well on
the decision values, the predictors have low complexity in the CCA
coordinate system: if $\lambda_i$ is large, minimizing the discrepancy encourages 
 $\tw^i$ to be close to $\lambda_i \tv^i$, and if $\lambda_i$ is small,
 minimizing the discrepancy encourages $\tw^i$ to be small (close to $0$). 
For any predictor $\vv$ of view $\z$, we defined the operator $T_{CCA} (\vv)$ to return a
corresponding predictor of view $\x$:
\begin{align*}
T_{CCA} (\vv) = \tU \cdot [\lambda_i (\tV^\top \vv)^i ]_{i=1}^{d_x}.
\end{align*}


\subsubsection{Multi-view knowledge distillation}
\label{sec:multiview-distill}

Similar to the distillation framework analyzed in previous section, we can
perform a two-step distillation process with multi-view data. In the first step, we train a
predictor $\hv$ based on labeled  data from the second view $\z$. And in
the next step, we train a predictor on labeled data from the first view
$x$, incorporating the soft supervision provided by $\hv$. Note that the
labeled data from each view need not overlap.

As before, we make the similar assumption that $\hv$ is learned from the
hypothesis class $\calC_v = \cbr{\vv: \norm{\vv}\le B_v}$ by performing ERM, 
with optimistic rate convergence due to low optimal expected loss $L_v^* = \min_{\vv
  \in \calC_v}\, L(\vv)$.
Since this view uses priviledged information (richer information),
learning is easy and a low-complexity hypothesis class (\eg, $B_v$ is small) suffices to achieve
low expected loss. 

Additionally, assume the optimal predictor $\w^*$ from the hypothesis class $\calC_w =
\cbr{\w: \norm{\w}\le B}$ agrees well with $\hv$ on decision values,
\ie, there exists some small $S>0$, such that 
\begin{align} \label{e:agreement-assumption-multiview}
\bbE \norm{{\w^*}^\top \x - \hv^\top \z}^2\le S^2. 
\end{align}
The following lemma provides an example when this assumption is satisfied.
\begin{lem}\label{lem:agreement-multiview}
Let the instantaneous loss $\ell(\cdot, \cdot)$ be $\lambda$-strongly convex
in the first argument. 
Let $\vv$ be a predictor from $\calC_v$ with $B_v \le B_w$, with expected
loss $L (T_{CCA} (\vv)) = \bbE \sbr{\ell \rbr{(T_{CCA}    (\vv))^\top \x, y}}$. 
Then we have
\begin{gather*}
\norm{\w^* - T_{CCA}  (\vv) }^2 = \bbE \norm{{\w^*}^\top \x -
  (T_{CCA}  (\vv))^\top \z }^2 \le \frac{2 (L (T_{CCA} (\vv)) -  L_w^*) }{\lambda}, \\
\text{and}\qquad\  \bbE \norm{{\w^*}^\top \x - \vv^\top \y }^2 \le
\frac{2(L (T_{CCA} (\vv)) -  L_w^*)}{\lambda} +  (1-\lambda_{d_z}) B_v^2.
\end{gather*}
where the expectation is taken over the data distribution.
\end{lem}
\begin{align*}
\end{align*}
\begin{proof}
The proof is similar to that of Lemma~\ref{lem:agreement}. 
By the definition of $T_{CCA}$, and the fact that $\lambda_i \le 1$, we
have that $\norm{T_{CCA} (\hv)} \le \norm{\hv} \le B_v \le B_w$.
Now that both $\w^*$ and $T_{CCA} (\vv)$ are in $\calC_w$ and $\w^*$ is
the minimizer of $L(\w)$ in $\calC_w$, we can use
the same argument in Lemma~\ref{lem:agreement}  and have
\begin{align*}
L (T_{CCA}(\vv)) - L (\w^*) \ge \frac{\lambda}{2}
  \norm{(T_{CCA}(\vv))^\top \x - {\w^*}^\top \x }^2.
\end{align*}
By our assumption of $\Exx=\I$, it holds that $\norm{(T_{CCA}(\vv))^\top \x -
  {\w^*}^\top \x }^2 = \norm{T_{CCA}  (\vv) - \w^*}^2$ and the first inequality follows.

To show the second inequality, just observe from
Lemma~\ref{lem:agreement-as-regularizer} that 
\begin{align*}
\bbE \norm{\w^\top \x - \vv^\top \z} & = \norm{\w - T_{CCA}(\vv)}^2
  +\sum_{i=1}^{d_z} (1-\lambda_i)^2 (\tv^i)^2 \\
& \le \norm{\w - T_{CCA}(\vv)}^2
  + (1-\lambda_{d_z})^2 \sum_{i=1}^d (\tv^i)^2 \\
&  \le \norm{\w - T_{CCA}(\vv)}^2
  + (1-\lambda_{d_z})^2 \norm{\vv}^2.
\end{align*}
\end{proof}
The following Theorem is completely analogous to
Theorem~\ref{thm:distill-rerm}.
\begin{thm} \label{thm:distill-rerm-multiview-1}
Compute either of the following predictors 
\begin{align} 
\label{e:distill-rerm-multiview-1}
& \hw = \argmin_{\w \in \calC_w}\; \frac{1}{n} \sum_{i=1}^n \ell (\w^\top
  \x_i, y_i)  + \frac{\nu}{2} \norm{\w - T_{CCA}(\hv)}^2 \\
\label{e:distill-rerm-multiview-2}
\text{or}\qquad
& \hw = \argmin_{\w \in \calC_w}\; \frac{1}{n} \sum_{i=1}^n \ell (\w^\top
  \x_i, y_i)  + \frac{\nu}{2} \bbE_{\x,\z} \norm{\w^\top \x - \hv^\top \z}^2
\end{align}
with $\nu=\frac{8\beta R^2}{n} + \sqrt{\frac{64\beta^2 R^4}{n^2} +
  \frac{16\beta R^2 L_w^*}{n S^2}}$. 
The we have
\begin{align*}
\bbE \sbr{L(\hw) - L_w^*} \le \frac{16 \beta R^2 S^2}{n} +
  \sqrt{\frac{16\beta R^2 L_w^*
  S^2}{n}}.
\end{align*}
\end{thm}
The difference in the two predictors is that~\eqref{e:distill-rerm-multiview-2} does not require computing
$T_{(CCA)} (\hv)$ (or the CCA system). 

Similar to single-view distillation case, the additional complexity
control from the multi-view agreement assumption allows us to reduce the
search space and achieve faster convergence. 
In particular, when the assumptions of Lemma~\ref{lem:agreement-multiview}
holds, the predictor~\ref{e:distill-rerm-multiview-1}
achieves the convergence rate
\begin{align*}
L (\hw) - L_w^* = \calO \rbr{ \frac{\beta R^2 (L(T_{CCA}(\hv)) -
  L_w^*)}{\lambda n} + \sqrt{\frac{\beta R^2 L_w^* (L(T_{CCA}(\hv)) -
  L_w^*)}{\lambda n}} }
\end{align*}
as opposed to % $\calO \rbr{\frac{\beta R^2 B_w^2}{n} + \sqrt{\frac{\beta  R^2  L_w^*}{n}} }$. 
The low expected error of $L(T_{CCA}(\hv)) $ measure how well the
priviledged information can be transfered. 

Kakade assumed that both views are powerful enough to learn the class
well, we assume only the transformed predictor works well in view $x$,
they need not be the same order. whereas $L_v^*$ can be much lower than $L_w^*$. 

Vapnik and Lopez et al focused on learning with 0-1 loss where the
complexity of hypothesize class is controlled with its VC-dimension, while
we study the generalized PAC learning.
We generalize Kakade's analysis for least squares.

For the least squares loss, \citet{KakadeFoster07a} propose to use $\sbr{ \frac{\lambda_i}{n} \sum_{j=1}^n \x^i_j \y_j }$ (dubbed the ``canonical shrinkage estimator''), which corresponds to the solution to the ERM objective regularized by a special ``canonical norm''.\footnote{Strictly speaking, it is not a norm if any $\lambda_i=0$ or $1$.} 
The authors showed that the shrinkage estimator has lower variance than the non-regularized ERM solution, while having similar bias. Their analysis relied heavily on the closed-form solution for least squares.


\subsection{Multi-task learning of two predictors simultaneously}
In the previous subsection, we still require first learning the view \z
\message{ !name(algorithm1.tex) !offset(-164) }


==> conclusion.tex <==
\section{Lower bound}
\label{sec:lower-bound}
\vspace*{-1ex}

Consider the following Gaussian distribution named \emph{single canonical pair model}~\citep{Chen_13e}:
\begin{align} \label{e:lower-bound-cov}
\left[\begin{array}{c}\x \\ \y\end{array}\right] \sim 
\calN \left(\0, \, \left[
\begin{array}{cc}
\I & \Delta  \bphi \bpsi^\top  \\
\Delta \bpsi \bphi^\top &  \I 
\end{array} 
\right]  \right),
\end{align}
where $\norm{\bphi}=\norm{\bpsi} = 1$. 
It is straightforward to check that $\T = \Exy = \Delta \bphi \bpsi^\top$ for such a distribution. Observe that $\T$ is of rank one and has a singular value gap $\Delta$, and the single pair of canonical directions are $\left( \uu^*, \vv^* \right) = \left(  \bphi,\, \bpsi \right)$. Denote this class of model by $\calF (d_x, d_y, \Delta)$. 
We have the following minimax lower bound for CCA under this model, which is an application of the result of~\citet{Gao_15a} for sparse CCA (by using rank $r=1$ and hard sparsity, \ie, $q=0$ and sparsity level $d$ in their Theorem~3.2). 

\begin{lem}[Lower bound for single canonical pair model]
Suppose the data is generated by the single canonical pair model. Let $(\uu,\, \vv)$ be some estimate of the canonical directions $(\uu^*,\, \vv^*)$ based on $N$ samples. Then, there is a universal constant $C$, so that for $N$ sufficiently large, we have:
\begin{align*}
\inf_{\uu,\vv}\; \sup_{ \stackrel{\uu^*,\vv^* \in }{\calF (d_x, d_y, \Delta)}} \; \bbE \left[ 1 - \text{align} \left( (\uu_T, \vv_T); (\uu^*, \vv^*) \right) \right] \ge C \frac{d}{\Delta^2 N}.
\end{align*}
\end{lem}

This lemma implies that, to estimate the canonical directions up to $\epsilon$-suboptimality in our measure of alignment, we expect to use at least $\calO \left( \frac{d}{\epsilon \Delta^2} \right)$ samples. 
We therefore observe that, for Gaussian inputs, the sample complexity of the our streaming algorithm matches that of the minimax rate of CCA, up to small factors.

